Demo -- Zelig: Customizable Blockchain Simulator

As blockchain-based systems see wider adoption, it becomes increasingly critical to ensure their reliability, security, and efficiency. Running simulations is an effective method of gaining insights on the existing systems and analyzing potential improvements. However, many of the existing blockchain simulators have various shortcomings that yield them insufficient for a wide range of scenarios. In this demo paper, we present Zelig: our blockchain simulator designed with the main goals of customizability and extensibility. To the best of our knowledge, Zelig is the only blockchain simulator that enables simulating custom network topologies without modifying the simulator code. We explain our simulator design, validate via experimental analysis against the real-world Bitcoin network, and highlight potential use cases.

==> tables/bitcoin_stats.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
         \hline
         \textbf{Region} & \textbf{Down} (MB/s) & \textbf{Up} (MB/s) & \textbf{Nodes} & \textbf{Mine Power} (\%) \\ \hline
         China           & 31.6                 & 23.6               & 189            & 65.08  \\ \hline
         US              & 55.3                 & 19.2               & 1,892          & 7.24   \\ \hline
         Russia          & 23.1                 & 20.2               & 251            & 6.90   \\ \hline
         Kazakhstan      & 12.9                 & 8.0                & 5              & 6.17   \\ \hline
         Malaysia        & 25.1                 & 19.4               & 19             & 4.33    \\ \hline
         Canada          & 59.0                 & 14.6               & 316            & 0.82    \\ \hline
         Germany         & 63.4                 & 24.5               & 1,769          & 0.56    \\ \hline
         Norway          & 37.5                 & 17.6               & 32             & 0.48    \\ \hline
         Venezuela       & 7.7                  & 3.5                & 2              & 0.42    \\ \hline
         \textbf{TOTAL}  & -                    & -                  & 4,475          & 92.0      \\ \hline
    \end{tabular}
    \vspace{0.1cm}
    \caption{Real world bandwidth, node count, and mine power distribution statistics for the Bitcoin network.}
    \label{tab:btc_stats}
\end{table}

==> tables/languages.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Paper} & \textbf{Language} & \textbf{Code} \\ \hline
         \cite{alharby_blocksim_2020} &  Python &  \href{https://github.com/maher243/Blocksim}{https://github.com/maher243/Blocksim}
        \\ \hline
         \cite{aoki_simblock_2019} & Java &  \href{https://github.com/dsg-titech/simblock}{https://github.com/dsg-titech/simblock}
        \\ \hline
         \cite{faria_blocksim_nodate} & Python & \href{https://github.com/carlosfaria94/blocksim}{https://github.com/carlosfaria94/blocksim}
        \\ \hline
         \cite{gervais_security_2016} & C++ & \href{https://github.com/arthurgervais/Bitcoin-Simulator}{https://github.com/arthurgervais/Bitcoin-Simulator}
        \\ \hline
         \cite{pandey_blocksim_nodate} & Python & \href{https://github.com/RoseBay-Consulting/BlockSim}{https://github.com/RoseBay-Consulting/BlockSim}
        \\ \hline
         \cite{stoykov_demo_nodate} & Scala & \href{https://github.com/i13-msrg/vibes/}{https://github.com/i13-msrg/vibes/} 
        \\ \hline 
    \end{tabular}
    
    \vspace{0.1cm}
    \caption{Programming languages the selected simulators are implemented in, and links to their source codes.}
    \label{tab:languages}
\end{table}

==> tables/properties_table.tex <==

\begin{table*}[t!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        \textbf{Features}&        
        Blocksim- & Simblock \cite{aoki_simblock_2019} & Blocksim- & Gervais- & Blocksim- & VIBES \cite{stoykov_demo_nodate} & \textbf{Our Work}\\ 
        & Alharby \cite{alharby_blocksim_2020} &  & Faria \cite{faria_blocksim_nodate} & Simulator \cite{gervais_security_2016} & Pandey \cite{pandey_blocksim_nodate} & &  \\ \hline
        Block size distribution                 &            &            &           & \checkmark &             &             & \checkmark \\ \hline
        Geographic network conditions           &            & \checkmark & \checkmark& \checkmark &             &             & \checkmark   \\ \hline
        Information propagation mechanism       &            &\checkmark  & \checkmark& \checkmark &             &             & \checkmark  \\ \hline
        Compare real time and simulation time   &            &\checkmark  &           & \checkmark &             &             & \checkmark  \\ \hline
        Consensus algorithms besides PoW        &            &            &           &            &             &             &             \\  \hline
        Block interval distribution             &            &            &           & \checkmark &             &             & \checkmark     \\ \hline
        Dynamic mining difficulty               &            &            &           &            &             &             &    \\ \hline
        Transaction fees                        & \checkmark &            &           &            &             &  \checkmark & \checkmark * \\ \hline
        Transaction modeling                    & \checkmark &            & \checkmark&            &  \checkmark &  \checkmark & \checkmark *  \\ \hline
        % \multicolumn{7}{|c|}{\textbf{Outputs}} \\ \hline 
        % Transactions per second             & \checkmark &            &           &            & \checkmark &  \checkmark \\ \hline
        % Cost per transaction                &            &            &           &            &            &  \checkmark \\ \hline
        % Block/transaction propagation delay &            & \checkmark & \checkmark& \checkmark & \checkmark &  \checkmark \\ \hline
        % Stale block rate                    & \checkmark & \checkmark &           & \checkmark &            &  \checkmark \\ \hline
        % Security parameters                 &            & \checkmark &           & \checkmark &            &  \checkmark \\ \hline
    \end{tabular}
    \vspace{0.1cm}
    \caption{Input and output parameters available for the selected simulators. Checkmarks correspond existing features. Empty cells either correspond to fixed values being assumed, or missing features ($*$: partially implemented).}
    \label{tab:inputs_outputs}
\end{table*}
